Meta Dropout: Learning to Perturb Features for Generalization

A machine learning model that generalizes well should obtain low errors on unseen test examples. Thus, if we know how to optimally perturb training examples to account for test examples, we may achieve better generalization performance. However, obtaining such perturbation is not possible in standard machine learning frameworks as the distribution of the test data is unknown. To tackle this challenge, we propose a novel regularization method, meta-dropout, which learns to perturb the latent features of training examples for generalization in a meta-learning framework. Specifically, we meta-learn a noise generator which outputs a multiplicative noise distribution for latent features, to obtain low errors on the test instances in an input-dependent manner. Then, the learned noise generator can perturb the training examples of unseen tasks at the meta-test time for improved generalization. We validate our method on few-shot classification datasets, whose results show that it significantly improves the generalization performance of the base model, and largely outperforms existing regularization methods such as information bottleneck, manifold mixup, and information dropout.

==> maintable2.tex <==
\begin{table}[t]
	\begin{center}
		\small
		\begin{tabular}{ccc}
			\toprule
			Models & Omniglot & mini-ImageNet \\
			& 20-way & 5-way \\
			\hline
			\hline
			Meta-SGD \cite{meta_sgd} & 95.93 $\pm$ 0.38 & 50.47 $\pm$ 1.87 \\
			Prob. MAML \cite{prob_maml} & - & 50.13 $\pm$ 1.86 \\
			MAML + indep. noise & 94.61 $\pm$ 0.17 & 47.54 $\pm$ 0.63 \\
			\hline
			Meta Dropout (MAML) & \bf 96.55 $\pm$ 0.14 & \bf 50.92 $\pm$ 0.66 \\ %\bf65.23 $\pm$ 0.52 \\
			\bottomrule	
		\end{tabular}
		\vspace{0.05in}
		\caption{\small 1-shot classification performance of other baselines.}\label{tbl:fsl2}
	\end{center}
	\small
\end{table}

==> table_adv.tex <==
\begin{table}[h]
	\begin{center}
		\small
		\caption{\small \textbf{Ablation study on the noise type}}
		\begin{tabular}{ccccc}
			\toprule
		 &\multicolumn{2}{c}{Omniglot 20-way} & \multicolumn{2}{c}{miniImageNet 5-way} \\
			Models & 1-shot & 5-shot & & \\
			\hline
			\hline
			MAML & 95.23\tiny$\pm$0.17 & 98.38\tiny$\pm$0.07 & 49.58\tiny$\pm$0.65 & 64.55\tiny$\pm$0.52 \\
			MAML + FG & xx.xx\tiny$\pm$x.xx & xx.xx\tiny$\pm$x.xx & xx.xx\tiny$\pm$x.xx & xx.xx\tiny$\pm$x.xx \\
			MAML + IG & xx.xx\tiny$\pm$x.xx & xx.xx\tiny$\pm$x.xx & xx.xx\tiny$\pm$x.xx & xx.xx\tiny$\pm$x.xx \\
			\hline
			Deterministic Meta-dropout & 95.99\tiny$\pm$0.14 & 98.29\tiny$\pm$0.07 & 50.75\tiny$\pm$0.63 & 65.62\tiny$\pm$0.53 \\
			Meta-dropout & \bf 96.63\tiny$\pm$0.13 & \bf 98.72\tiny$\pm$0.07 & \bf 51.93\tiny$\pm$0.67 & \bf 67.42\tiny$\pm$0.52 \\
			\bottomrule	
		\end{tabular}
	\end{center}
\end{table}

==> table_resnet.tex <==
\begin{table*}
	\begin{center}
		\caption{\small \textbf{Few-shot classification performance} on ResNet-12 or WRN28-10 architectures. All reported results are average performances over 1000 randomly selected episodes with standard errors for 95\% confidence interval over tasks.}\label{tbl:resnet}
		\vspace{-0.05in}
		\small
		\resizebox{\textwidth}{!}{
		\begin{tabular}{cccccc}
			\toprule
			& &\multicolumn{2}{c}{miniImageNet 5-way} & \multicolumn{2}{c}{tieredImageNet 5-way} \\%\cmidrule{1-5}
			Models & Backbone & 1-shot & 5-shot & 1-shot & 5-shot \\
			\hline
			\hline
			SNAIL~\citep{snail} & ResNet-12 & 55.71\tiny$\pm$0.99 & 68.88\tiny$\pm$0.92 & - & - \\
			AdaResNet~\citep{adaresnet} & ResNet-12 & 56.88\tiny$\pm$0.62 & 71.94\tiny$\pm$0.57 & - & - \\
			TADAM~\citep{tadam} & ResNet-12 & 58.50\tiny$\pm$0.30 & 76.70\tiny$\pm$0.30 & - & - \\
			Activation to Parameter~\citep{act2param} & WRN28-10 & 59.60\tiny$\pm$0.41 & 73.74\tiny$\pm$0.19 & - & - \\
			Prototypical Networks~\citep{protonet} & ResNet-12 & 59.25\tiny$\pm$0.64 & 75.60\tiny$\pm$0.48 & 61.74\tiny$\pm$0.77 & 80.00\tiny$\pm$0.55 \\
			LEO~\citep{leo} & WRN28-10 & 61.76\tiny$\pm$0.61 & 77.59\tiny$\pm$0.12 & 66.33\tiny$\pm$0.05 & 81.44\tiny$\pm$0.09 \\
			MetaOptNet~\citep{metaoptnet} & ResNet-12 & 62.64\tiny$\pm$0.61 & 78.63\tiny$\pm$0.46 & 65.99\tiny$\pm$0.72 & 81.56\tiny$\pm$0.53 \\
			\hline
			%MAML (ours) & ResNet-12 & \bf 63.74\tiny$\pm$1.42 & 78.14\tiny$\pm$1.29 & xx.xx & xx.xx \\
			%MAML + Meta-dropout & ResNet-12 & 63.02\tiny$\pm$1.55 & \bf 79.54\tiny$\pm$1.25  & xx.xx & xx.xx \\
			MAML (our reproduction) & ResNet-12 & 59.62\tiny$\pm$0.74 & 74.12\tiny$\pm$0.55 & xx.xx & xx.xx \\
			\bf MAML + Meta-dropout & ResNet-12 & 59.66\tiny$\pm$0.72 & \bf xx.xx\tiny$\pm$x.xx & xx.xx & xx.xx \\
						%MAML (our reproduction) & ResNet-12 & 63.00\tiny$\pm$1.44 & 78.42\tiny$\pm$1.34 & xx.xx & xx.xx \\
			\bf MAML + Meta-dropout & ResNet-12 & 63.06\tiny$\pm$1.49 & \bf 79.98\tiny$\pm$1.26 & xx.xx & xx.xx \\
			
			\hline
			\bottomrule	
		\end{tabular}
	}
	\end{center}
	\small
\end{table*}

